Case study: Class diagram restructuring

This case study is an update-in-place refactoring transformation on UML class diagrams. Its aim is to remove clones of attributes from a class diagram, and to identify new classes which abstract groups of classes that share common data features. It is used as one of a general collection of transformations (such as the removal of redundant inheritance, or multiple inheritance) which aim to improve the quality of a specification or design level class diagram. The transformation is a typical example of a model refactoring, and illustrates the issues involved in such transformations.

==> eptcsdata.tex <==
\providecommand{\firstpage}{8}
\providecommand{\publicationstatus}{Pieter Van Gorp, Louis M. Rose, Christian Krause (Eds.):\\
Sixth Transformation Tool Contest (TTC 2013)\\
EPTCS 135, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.135.2}{10.4204/EPTCS.135.2}}

